Observation of coherent coupling between super- and subradiant states of an ensemble of cold atoms collectively coupled to a single propagating optical mode

We discuss the evolution of the quantum state of an ensemble of atoms that are coupled via a single propagating optical mode. We theoretically show that the quantum state of N atoms, which are initially prepared in the timed Dicke state, evolves through all the N - 1 states that are subradiant with respect to the propagating mode. We predict this process to occur for any atom number and any atom-light coupling strength. These findings are supported by measurements performed with cold cesium atoms coupled to the evanescent field of an optical nanofiber. We experimentally observe the evolution of the state of the ensemble passing through the first two subradiant states, leading to sudden, temporary switch-offs of the optical power emitted into the nanofiber. Our results contribute to the fundamental understanding of collective atom-light interaction and apply to all physical systems, whose description involves timed Dicke states.

==> ArXiv Submission/0_Abstract.tex <==
We discuss the evolution of the quantum state of an ensemble of atoms that are coupled via a single propagating optical mode. We theoretically show that the quantum state of $N$ atoms, which are initially prepared in the timed Dicke state, evolves through all the $N-1$ states that are subradiant with respect to the propagating mode.
%, eventually remaining in a superposition of the timed Dicke- and the subradiant states with equal probability
We predict this process to occur for any atom number and any atom--light coupling strength. These findings are supported by measurements performed with cold cesium atoms coupled to the evanescent field of an optical nanofiber. We experimentally observe the evolution of the state of the ensemble passing through the first two subradiant states, leading to sudden, temporary switch-offs of the optical power emitted into the nanofiber. Our results contribute to the fundamental understanding of collective atom--light interaction and apply to all physical systems, whose description involves timed Dicke states.



==> ArXiv Submission/1_Introduction.tex <==


%\section{Introduction}

The collective interaction of $N$ quantum emitters with light can differ substantially depending on whether the distance between any two of the emitters is significantly smaller or larger than the wavelength of the light field.
The former situation has been initially investigated by Dicke \cite{Dicke1954}, who decomposed the Hilbert space of the system in superradiant states, whose decay rate towards lower energy states is enhanced with respect to the one of an isolated emitter, and subradiant states, for which decay to the ground state is suppressed. In particular, in the single excitation limit which we consider throughout this Letter, the Dicke model identifies a single superradiant state with an $N$ times enhanced decay rate, while there are $N-1$ subradiant states.

A formal description of the time evolution of extended ensembles of emitters 
(i.e., inter-atomic distance between any two emitters $> \lambda$) 
within the same framework of the Dicke model requires the introduction of the so-called timed Dicke states \cite{Scully2006}, which can be prepared, e.g., by exciting the emitters with a single photon with wavevector $\boldsymbol{k}$:
\begin{eqnarray}
\ket{\textrm{TD}} = \dfrac{1}{\sqrt{N}} \sum_{n=1}^{N}  e^{i \boldsymbol{k} \cdot \boldsymbol{r}_\textbf{\textit{n}}} \hat{\sigma}^+_n \ket{0} ~.
\label{eq:TimedDickeState}
\end{eqnarray}
Here, $\boldsymbol{r}_\textbf{\textit{n}}$ and $\hat{\sigma}^+_n$ indicate the position and the raising operator for the $n^\textrm{th}$ emitter in the ensemble and $\ket{0}=\ket{0_\textrm{ph}}\otimes \ket{g_1, ..., g_N}$, where $\ket{0_\textrm{ph}}$ is the vacuum state and $\ket{g_1, ..., g_N}$ indicates that all atoms are in the ground state.  An ensemble in the timed Dicke state experiences superradiant decay and collectively enhanced emission of light into the same optical mode that excited the system. Likewise, it is possible to introduce $N-1$ states, that are orthogonal to the timed Dicke state and subradiant with respect to the optical mode with wavevector $\boldsymbol{k}$.
This approach is suitable for describing a considerable number of physical systems, including for instance cold atom clouds \cite{Araujo2016, Roof2016, Guerin2016, Ferioli2021, Goban2015, Okaba2019, Bettles2020, Pennetta2021}, Rydberg atoms \cite{ParisMandoki2017, Stiesdal2020} and emitters in solid state samples \cite{Rohlsberger2010}.
In addition, in cavity quantum electrodynamics the timed Dicke physics is at the basis of the assumptions of the Tavis-Cummings model \cite{Tavis1968, Blaha2021}, which describes collectively enhanced light-matter coupling between an atomic ensemble and a single mode cavity \cite{Colombe2007, Brennecke2007}.
For these reasons, notable effort has been recently devoted to describe the time dynamics of extended ensembles \cite{Scully2006, Svidzinsky2008, Kumlin2020, Jen2020, Berman2020, Pivovarov2021}, a task which, unlike the standard Dicke model, needs to consider coupling between super- and subradiant states, see Fig. \ref{fig:PhysicalSetting}(a).




\begin{figure}[]
\includegraphics[width=0.95\linewidth]{Figures/PhysicalSetting.png}
\caption{\label{fig:PhysicalSetting} (a) Collective states for an ensemble of $N$ atoms in the single excitation limit. TD: timed Dicke state, sub$_n$: $n^\textrm{th}$ subradiant state, g: ground state. (b) $N$ atoms coupled to a single-mode optical waveguide. The factors $\beta_n \, 2\gamma$ and $ (1-\beta_n) \, 2\gamma$ represent the photon emission rate of the $n^\textrm{th}$ atom into guided and unguided optical modes, respectively. The excited state amplitude of the $n^\textrm{th}$ atom is indicated by $\phi_n$, while $\chi_n$ is the light field amplitude right after the $n^\textrm{th}$ atom. 
}
\end{figure}



In this Letter, we study % the paradigmatic setting of 
a one-dimensional ensemble of atoms coupled via a single optical mode, and we discuss the time evolution of its state.
We present a theoretical approach that unveils the microscopic % (i.e., atom per atom)
temporal dynamics of the system within a simple mathematical framework. We show that during its temporal evolution, an ensemble initially prepared in the timed Dicke state evolves through all basis states of the Hilbert space, reaching, one after the other, all the $N-1$ subradiant states.
This process occurs for any atom number (unlike the case of three-dimensional atom clouds \cite{Svidzinsky2008}) and for any coupling strength. Notably, it already appears for two emitters with arbitrarily weak coupling to the optical mode \cite{Kien2017}.
To support the predictions of our model, we present experimental results that we obtain interfacing an ensemble of cold cesium (Cs) atoms with the evanescent field part of the guided-mode of an optical nanofiber. After exciting the atoms with boxcar-shaped nanofiber-guided laser pulses with a switch-off time much shorter than the atomic lifetime, we investigate the temporal response of the system by recording the optical power exiting the nanofiber.
We observe the passage of the state of the ensemble through the first two subradiant states with respect to the guided mode, which leads to abrupt and temporary drops in the nanofiber-guided light field.



==> ArXiv Submission/2_Theory.tex <==
%\section{Theory}

%\subsection{Theory, model and solutions}

A sketch of the considered configuration is shown in Fig.~\ref{fig:PhysicalSetting}(b).
An ensemble of $N$ atoms %with inter-atomic distance $\gg \lambda$
is coupled to a single guided optical mode. The atom-waveguide coupling strength is characterized by the parameter $\beta_{n}$, defined as the ratio between the spontaneous emission rate of the $n^\textrm{th}$ atom into the considered waveguide mode and the total photon emission rate of a single-atom into all modes, $2 \gamma$, see Fig.~\ref{fig:PhysicalSetting}(b). Throughout this Letter, we assume unidirectional propagation, an approximation which is justified by the collective enhancement of forward emission typical of the timed Dicke state \cite{Scully2006, Pennetta2021} and which holds as long as the atoms are not arranged at the Bragg condition (i.e., inter-atomic distance equal to an integer multiple of $\frac{\lambda}{2}$). In addition, for simplicity we also assume that all atoms have the same coupling strength $\beta$ to the waveguide, a situation which describes well, e.g., trapped atoms \cite{Vetsch2010, Thompson2013, Goban2015}. However, our model can be easily extended to the general case, as shown in the Supplemental Material.
%indeed, while the system considered is only partially chiral \cite{Lodahl2017}, this approximation is justified by the collective enhancement of forward emission typical of the timed Dicke state \cite{Scully2006, Pennetta2021}(a part for atoms distributed at the Bragg condition, needed?).

The general quantum state of the system can be written as:
\begin{align}
\nonumber
\ket{\psi(t)} =& \bigg[ \sum_{n=1}^N e^{ik z_n}\phi_n(t)\hat{\sigma}^+_n +
\\
&+ \int_{-\infty}^{\infty} e^{ik z_n} \chi(t,z) \hat{a}_z^{\dagger} dz \bigg] \ket{0} +
\ket{\psi_{fs}(t)} ~,
\label{eq:GeneralState}
\end{align}
where $\phi_n(t)$ and $z_n$ represent the excited state amplitude and the position along the fiber of the $n^\textrm{th}$ atom in the ensemble, respectively. In addition, $\chi(t,z)$ indicates the complex amplitude of the waveguide-coupled light field, $\hat{a}_z^{\dagger}$ is the creation operator for a forward-propagating photon at position $z$, and $\ket{\psi_{fs}(t)}$ denotes the state of the photons that are emitted into free space.

The collective decay rate of the ensemble, $\Gamma_{ens}(t)$, is defined as the ratio between the energy loss rate and the energy stored in the ensemble:
\begin{eqnarray}
\Gamma_{ens}(t) = - \frac{\sum_{n=1}^{N} \tfrac{\partial}{\partial t} \lvert\phi_n(t) \rvert^2 }{\sum_{n=1}^{N} \lvert\phi_n(t) \rvert^2 } = \Gamma_{fs} + \Gamma_{ens, wg}(t) ~,
\label{eq:Gamma_coll}
\end{eqnarray}
where $\Gamma_{fs}=(1-\beta)2\gamma$ is the decay rate into free space, that we assume to be the same for all atoms. The second term, $\Gamma_{ens, wg}(t)$, indicates the ensemble decay rate into the waveguide, defined as the energy leaving the ensemble via guided light divided by the stored energy:
\begin{eqnarray}
\Gamma_{ens, wg}(t) = 
%2\beta \gamma \frac{\lvert \sum_{n=1}^{N} \phi_n(t) \rvert^2 }{\sum_{n=1}^{N} \lvert\phi_n(t) \rvert^2 } = 
\frac{ v_g \lvert \chi_N(t) \rvert^2 }{\sum_{n=1}^{N} \lvert\phi_n(t) \rvert^2 } ~,
\label{eq:Gamma_coll_wg}
\end{eqnarray}
where $\chi_{N}(t)$ is the complex amplitude of the light field right after the $N^\textrm{th}$ atom and  $v_g$ is the group velocity of the guided optical mode.
We note that  $\Gamma_{ens}(t)$ is sometimes inferred from the decay rate of the light intensity emitted by the atoms into the considered mode, $\Gamma_{light}(t)$, \cite{Guerin2016, Bettles2020, Roof2016, Stiesdal2020, Pennetta2021}, i.e.:
%$d(\textrm{log}(|\chi(t)|^2/|\chi(0)|^2)/dt$ 
\begin{equation}
\Gamma_{light}(t)=-\dfrac{\partial}{\partial t} \left[ \textrm{log} \left( \dfrac{|\chi_N(t)|^2}{|\chi_N(0)|^2} \right) \right] = - \frac{ \tfrac{\partial}{\partial t} \lvert \sum_{n=1}^{N} \phi_n(t) \rvert^2 }{\sum_{n=1}^{N} \lvert\phi_n(t) \rvert^2 } ~.
\label{eq:Gamma_light}
\end{equation}
However, while convenient to access experimentally, a comparison between Eqs.~(\ref{eq:Gamma_coll}) and (\ref{eq:Gamma_light}) shows that this quantity is in general not related to $\Gamma_{ens} (t)$, whose estimation requires access to the complete state of the system. Interestingly, $\Gamma_{ens}$ and $\Gamma_{light}$ coincide for the timed Dicke state.

To theoretically describe the time-evolution of $\ket{\psi(t)}$, we follow the approach of \cite{Shen2009, Blaha2021, Pennetta2021}, which, starting from a real-space Hamiltonian, allows us to calculate the excitation amplitudes, $\phi_n$, in the steady state by solving the time-independent Schr\"odinger equation. In the low excitation limit, the dynamics of the system in the time-domain can be then obtained via Fourier analysis (see Supplemental Material).

For a system that is prepared in the timed Dicke state, i.e., $\phi_n(t=0)=1/\sqrt{N}$, with $n=1,...,N$, and that then evolves freely, our model allows us to derive analytic expressions for $\phi_n(t)$ and $\chi_{n}(t)$, where the latter is proportional to the sum of the excited state amplitudes of the first $n$ atoms:
\begin{equation}
\phi_n(t) = \dfrac{1}{\sqrt{N}} e^{-\gamma t}L_{n-1}^{(0)}(2 \beta \gamma t) ~,
\label{eq:SolutionsTimedDickeStateAtoms}
\end{equation}
\begin{equation}
\chi_n(t) = \dfrac{\sqrt{2 \beta \gamma}}{i \sqrt{v_g}} \sum_{m=1}^n \phi_m(t) 
= \dfrac{\sqrt{2 \beta \gamma}}{i \sqrt{v_g N}}e^{-\gamma t}L_{n-1}^{(1)} (2 \beta \gamma t) ~,
\label{eq:SolutionsTimedDickeStateLight}
\end{equation}
where $L_{m}^{(\alpha)}$ are the generalized Laguerre polynomials.
%, which are polynomials of order $m$ with $m$ different zeros
The solutions show that, with the exception of the factor $e^{-\gamma t}$, the entire dynamics only depends on the product $\beta \gamma t$ and therefore it is essentially the same for any emitter-mode coupling strength, $\beta$, after appropriate scaling of the observation time. In the limit $\beta = 1$, these results agree with calculations based on a master equation approach \cite{Kumlin2020}.


%\subsection{Theory, properties of the solutions}

\begin{figure}[]
\includegraphics[width=0.95\linewidth]{Figures/Theory4Atoms.pdf}
%\includegraphics[width=0.95\linewidth]{Figures/4_Particles_Evolution.png}
\caption{\label{fig:Theory}
(a) Calculated waveguide-coupled power, $|\chi(t)|^2$, (normalized at $t=0$) as a function of time for $N=4$ atoms (blue line) with $\beta=0.4$. For comparison, the case for $N=1$ atom is shown as a gray line.
(b) Ensemble decay rate, $\Gamma_{ens}(t)$, as a function of normalized time. The vertical blue dashed lines indicate the instants corresponding to which the ensemble is in a subradiant state with respect to the waveguide, $t = \tau_i$, $i = 1, 2, 3$.
(c) Normalized excited state amplitude for the atoms in the ensemble for the timed Dicke state and the subradiant states.
(d) Projection on the timed Dicke state and the subradiant states of the residual excitation stored in the ensemble as a function of time.
}
\end{figure}


Equations~(\ref{eq:SolutionsTimedDickeStateAtoms}) and~(\ref{eq:SolutionsTimedDickeStateLight}) completely determine the state of the system and allow one to calculate quantities of interest such as the total waveguide-coupled optical power, $|\chi(t)|^2$, and $\Gamma_{ens}(t)$, which, as an example, are shown in Fig.~\ref{fig:Theory}(a) and (b), respectively, for the case $N=4$ and $\beta=0.4$.
At $t=0$ the ensemble is in the timed Dicke state and exhibits a superradiant decay rate into the waveguide mode, which is $N$ times enhanced with respect to the one of a single atom: $\Gamma_{ens,wg}(0) = N \cdot \beta \, 2\gamma$.
For $t>0$, unlike for the predictions of the standard Dicke model, the waveguide-coupled light power exhibits $N-1$  zeros, whose times of occurrence, $\tau_m$ ($m=1, ..., N-1$), are the roots of $L_{N-1}^{(1)} (2 \beta \gamma t)$. This relation explicitly defines a set of states, which are subradiant with respect to the waveguide:
\begin{eqnarray}
\ket{\textrm{sub}_\textrm{m}} = \sum_{n=1}^N e^{ik z_n}\phi_n(\tau_m)\hat{\sigma}^+_n \ket{0} ~.
\label{eq:SubradiantStates}
\end{eqnarray}
For these states, we have $\Gamma_{ens,wg}(\tau_m) = 0$. However, the emission into free space is unmodified, therefore $\Gamma_{ens} (\tau_m) = \Gamma_{fs}$, which is also the minimum total decay rate that can be obtained in the considered configuration, see Fig.~\ref{fig:Theory}(b).
 
Figure~\ref{fig:Theory}(c) shows the excited state amplitudes for the super- and subradiant states. For instance, for the first subradiant state, $\ket{ \textrm{sub}_1 }$, the first and last two atoms of the ensemble radiate in phase opposition, causing fully destructive interference of the waveguide-coupled light fields.
The subsequent subradiant states are characterized by a similar structure but the number of sub-ensembles that radiate with opposite phases increases progressively by one.
These states are all orthogonal to each other and to the timed Dicke state (i.e., the superradiant state). All together, these states form a complete basis of the subspace in which a single excitation is shared by the atoms, allowing a full description of the state of the ensemble (see Supplemental Material).


To shed further light on the system dynamics, Fig.~\ref{fig:Theory}(d) shows the decomposition onto this basis of the residual excitation stored in the atoms as a function of time. The ensemble, initially prepared in the timed Dicke state, passes through all the subradiant states and eventually remains (for $t \gg \tau_{N-1}$) in a superposition of the timed Dicke- and the subradiant states with equal probability of $1/N$. At this point, $\Gamma_{ens}(t)$ asymptotically converges to the single-atom decay rate, i.e., $2 \gamma$, see Fig.~\ref{fig:Theory}(b). This process remains qualitatively unaltered for any atom number $N$ and coupling strength $\beta$.

%\subsection{Theory, Bessel functions}

It is interesting to note that for $\beta \ll 1$ and large $N$ the time evolution of the ensemble becomes independent of the individual atom-mode coupling strength and only depends on the optical depth, OD $\simeq 4 \beta N$. Indeed, under these conditions, we can approximate Eqs.~(\ref{eq:SolutionsTimedDickeStateAtoms}) and~(\ref{eq:SolutionsTimedDickeStateLight}) as:
\begin{eqnarray}
\phi_n(t) \simeq & \dfrac{1}{\sqrt{N}} e^{-\gamma t} J_{0}\bigg( \sqrt{2 \gamma\, \textrm{OD}\, \frac{n-1}{N} t} \bigg) ~, \qquad
\label{eq:SolutionsTimedDickeStateAtomsBessel}
\end{eqnarray}
\begin{eqnarray}
\chi_N(t) \simeq & \dfrac{\sqrt{\textrm{OD}}}{i \sqrt{4v_g \beta t}}e^{-\gamma t} J_{1} (\sqrt{2 \gamma \, \textrm{OD} \, t}) ~, \quad
\label{eq:SolutionsTimedDickeStateLightBessel}
\end{eqnarray}
where $J_\alpha(x)$ are the Bessel functions of the first kind (see Supplemental Material). These relations are relevant for experiments involving large numbers of emitters and agree with results obtained for continuous resonant media \cite{Buerck1999}. The fact that the argument of the Bessel functions only depends on the OD suggests that the dynamics of the system is also well described by Eqs.~(\ref{eq:SolutionsTimedDickeStateAtomsBessel}) and (\ref{eq:SolutionsTimedDickeStateLightBessel}) when the coupling strength varies from atom to atom as long as $\beta_n\ll 1$, see Fig.~\ref{fig:PhysicalSetting}. We numerically confirmed that this is indeed the case.



==> ArXiv Submission/3_Experiment.tex <==
%\section{Experiment}

%\begin{figure}[]
%\includegraphics[width=1\linewidth]{Figures/SketchSetup.png}
%\caption{\label{fig:SketchSetup} Sketch of the exprimental setup. Cs: cesium, EOM: electro-%optic modulator, AOM: acousto-optic modulator, SPCM: single photon counting module.}
%\end{figure}

\begin{figure}[]
\includegraphics[width=.9\linewidth]{Figures/SketchSetup.png}
\includegraphics[width=.94\linewidth]{Figures/Exp_data.pdf}
\caption{\label{fig:Exp_data} (a) Experimental setup. Cs: cesium, EOM: electro-optic modulator, AOM: acousto-optic modulator, SPCM: single photon counting module. (b) Measured (blue dots) and predicted (red line) optical power exiting the nanofiber for $\Delta = 0$ and OD $=31$. The blue shaded area shows the measured pulse in the absence of atoms. (c) Measured (blue dots) and predicted (red line) homodyne signal between the atoms-emitted light and a local oscillator for the same parameters as in (b). (d, e) Calculated excited state amplitudes of each atom for the parameters as in (b) for the first (d) and second (e) subradiant state. These states are reached at $t=6.1$~ns and $t=30.6$~ns, as indicated in (b, c) with dashed gray lines. (f) Time at which the system reaches the first (blue line and dots), second (red line and dots) and third (green line and dot) subradiant states as a function of the OD. The measurements for OD of 42 and 63 have been obtained with multiple passes of the pulse through the ensemble, see Suppl. Mat. The dots are measured data, while the solid and dashed lines are theoretical predictions for $\beta = 0.55\%$ and $\beta = 20\%$, respectively. (g) Measured optical power for OD $=28$ and $\Delta$ = 1.1 $\gamma$ (blue dots), $\Delta$ = 2.3 $\gamma$ (red dots) and $\Delta$ = 4.6 $\gamma$ (green dots). The solid lines are theoretical predictions.
%The dots represent the measured data, while the solid lines illustrate our theoretical predictions. The blue shaded area shows the measured pulse shape in the absence of atoms.
}
\end{figure}

%\begin{figure}[]
%\includegraphics[width=1\linewidth]{Figures/Detuning_scan.pdf}
%\caption{\label{fig:Detuning_scan} (a-c) Measured transmitted optical power for an OD=28 and a detuning $\Delta$ of (a) 0.5 $\Gamma_0$, (b) 1.1 $\Gamma_0$ and (c) 2.3 $\Gamma_0$. The dots represent the measured data, while the solid lines illustrate our theoretical predictions. The gray shaded area shows the measured pulse shape in the absence of atoms. (d-f) Calculated excitation amplitude (left axis) and phase (right axis) for each of the atom in the ensemble for the same parameters of (a-c) respectively.}
%\end{figure}

%In the timed Dicke state all the atoms have uniform excitation amplitudes.

In the one-dimensional geometry considered here, the timed Dicke state can be approximately prepared by exciting the atoms with very short laser pulses, carrying an average energy corresponding to less than one photon. However, this method is very inefficient because most of the time the excitation pulse passes through the ensemble without interacting with the atoms, complicating the observation of the atom-emitted light with good signal to noise ratio.
To experimentally explore the concepts discussed above, we therefore preferred to employ long boxcar-shaped excitation pulses. They prepare a state, whose time dynamics has the same features of the one of the timed Dicke state but can be prepared with significantly higher probability, see Supplemental Material.

%The undesirable consequence of this approach is that only very little energy is stored in the ensemble, which complicates the observation of the atom emitted light with high signal to noise ratio.
%Increasing the intensity of the excitation pulse may result in saturation or damaging of the light detectors.
%For these reasons, to experimentally explore the concepts discussed above, we preferred to employ long boxcar-shaped excitation pulses, which prepare the ensemble in a state, whose time dynamics is qualitatively identical to the one of the timed Dicke state (see supplemental material), but allow to achieve significantly higher excited state populations.

%\subsection{Experimental setup}

Fig.~\ref{fig:Exp_data}(a) shows a sketch of the experimental setup. A single-mode optical nanofiber with a 400-nm diameter and a waist length of 1 cm is placed in a vacuum chamber and surrounded by a cloud of cold Cs atoms from a magneto-optical trap (MOT). Nanofiber-guided excitation pulses that are near-resonant with the Cs D2 transition ($6S_{1/2}$, $F=4 \rightarrow 6P_{3/2}, F^\prime=5$) are generated from an incident cw laser beam using an electro-optic modulator followed by an acousto-optic modulator. The $<1$-ns fall-time (90$\%$-10$\%$) of the pulses is much shorter than the lifetime of the excited state ($\tau$ = $1/2\gamma$ = 30.4 ns, $\gamma/2\pi$ = 2.6 MHz~[\onlinecite{Steck2019}]), while the total pulse length (100~ns $>$ 3$\tau$) is long enough for the system to approximately reach a steady state.
%The slow switch-off time of the AOM ($\approx$ 50 ns) permits to increase the extinction ratio offered by the EOM for longer time scales. 
The optical power transmitted through the nanofiber is measured using a single-photon counting module. We note that each excitation pulse has a mean power significantly smaller than one single photon energy per atomic lifetime. This ensures that, on average, less than one excitation is stored in the atomic ensemble.
%The experiment is performed by alternating a preparatory phase, in which Cs atoms are loaded into the MOT, and a probing phase, during which the MOT is released and 20 probe pulses are launched into the nanofiber. The experimental data shown in Fig. \ref{fig:Exp_data} have been obtained by averaging the results obtained over $\approx 10^5$ single experimental realization.

%\subsection{OD scan}

Time-resolved measurements of the emitted optical power are shown in Fig.~\ref{fig:Exp_data}(b) for probe pulses resonant with the atomic transition, i.e., detuning $\Delta=\omega - \omega_a=0$, where $\omega_a=0$ is the atomic resonance frequency, and for OD $=31$.
Right after the switch-off of the excitation pulse at $t=0$, the ensemble initially decays at a superradiant rate, reaching minima in transmission around $t = 6.1$~ns and $t = 30.6$~ns. Fig.~\ref{fig:Exp_data}(d, e) depicts the calculated excited state amplitudes for the atoms in the ensemble at these moments in time. Complete destructive interference of the light emitted from atoms into the guided mode is predicted, i.e., the ensemble is in a subradiant state with respect to the nanofiber-guided mode.

Our theoretical model predicts a change in the sign of the projection of the ensemble state on the timed Dicke state and thus of the emitted light field amplitude each time the system passes through one of the subradiant states. To experimentally investigate this feature, we repeat the measurement of Fig.~\ref{fig:Exp_data}(b), this time interfering the light emitted by the atomic ensemble with a local oscillator. The result is shown in Fig.~\ref{fig:Exp_data}(c), in which clear constructive and destructive interference with the local oscillator is observed before and after the first subradiant state respectively, in very good agreement with our predictions.

Fig.~\ref{fig:Exp_data}(f) illustrates the time at which the system is in the first (blue points and lines), second (red points and lines) and third (green point and lines) subradiant state as a function of the OD. The theoretical predictions shown as solid lines have been calculated for $\beta=0.55\%$, which is the average value measured in our experiment~[\onlinecite{Johnson2019}], while the dashed lines correspond to a much larger value of $\beta=20\%$ (approximately the highest $\beta$ that can be achieved in a nanofiber atom-interface \cite{Kien2005}). The close agreement between the two theory predictions and the experimental data confirms that for $N \gg 1$ the time evolution of the system depends on OD rather than on atom number.

%\subsection{Detuning scan}

%In order for the ensemble to completely evolve during time into the subradiant states, excitation via resonant optical pulses is required. Because of the dispersive response of the ensemble, detuned excitation%
Excitation via moderately detuned laser pulses results in an additional phase shift between subsequent atoms due to the dispersive response of the ensemble, which prevents complete destructive interference of the collective emission.
This was experimentally investigated by launching into the nanofiber pulses, whose central frequency is detuned with respect to the atomic transition. The results are shown in Fig.~\ref{fig:Exp_data}(g), in which the transmitted power for a time interval close to when the system reaches the first subradiant state is depicted for several detunings $\Delta$. 
As expected, compared to the case $\Delta=0$, larger detunings cause a gradual disappearance of the first minimum in the transmitted optical power.

%Fig. \ref{fig:Detuning_scan}(d-f) illustrates the calculated excitation amplitude and phase at t=6.1 ns for the atoms in the array, showing that for $\Delta\ne0\Gamma_0$ MHz the first and the second half of the ensemble do not radiate in perfect phase opposition.



==> ArXiv Submission/4_Conclusions.tex <==
%\section{Conclusions}

%(Suggestions for the conclusion paragraph are warmly welcomed)

In conclusion, we have shown that an ensemble of $N$ emitters prepared in the timed Dicke state with respect to a given propagating mode evolves through $N-1$ subradiant states.
This results in aperiodic switch-offs of the collectively emitted optical power. This non-monotonous decay originates from the dynamics induced by atom--atom coupling via propagating photons.
Our predictions are in excellent agreement with power and phase-sensitive measurements of the light emitted by an ensemble of Cs atoms coupled to the guided mode of an optical nanofiber.
%occurs because, for an extended ensemble, collective effects are not the same for all atoms, but gradually build up along the propagation direction of light, resulting in a unique time evolution for the excited state population of each of the atoms in the ensemble \cite{Pennetta2021}.
Beyond providing fundamental insight into collective atom--light coupling, our results are of direct relevance for systems whose dynamics involve timed Dicke states as, e.g., optical quantum memories \cite{Lvovsky2009, Simon2010} and atomic ensembles in cavity and waveguide quantum electrodynamics \cite{Mivehvar2021, Johnson2019, Goban2015}.


